Kick Back & Relax++: Scaling Beyond Ground-Truth Depth with SlowTV & CribsTV

Self-supervised learning is the key to unlocking generic computer vision systems. By eliminating the reliance on ground-truth annotations, it allows scaling to much larger data quantities. Unfortunately, self-supervised monocular depth estimation (SS-MDE) has been limited by the absence of diverse training data. Existing datasets have focused exclusively on urban driving in densely populated cities, resulting in models that fail to generalize beyond this domain. To address these limitations, this paper proposes two novel datasets: SlowTV and CribsTV. These are large-scale datasets curated from publicly available YouTube videos, containing a total of 2M training frames. They offer an incredibly diverse set of environments, ranging from snowy forests to coastal roads, luxury mansions and even underwater coral reefs. We leverage these datasets to tackle the challenging task of zero-shot generalization, outperforming every existing SS-MDE approach and even some state-of-the-art supervised methods. The generalization capabilities of our models are further enhanced by a range of components and contributions: 1) learning the camera intrinsics, 2) a stronger augmentation regime targeting aspect ratio changes, 3) support frame randomization, 4) flexible motion estimation, 5) a modern transformer-based architecture. We demonstrate the effectiveness of each component in extensive ablation experiments. To facilitate the development of future research, we make the datasets, code and pretrained models available to the public at https://github.com/jspenmar/slowtv_monodepth.

==> Figures/araug.tex <==
% Aspect ratio augmentation.

\subfloat[Original (16:9)]{\includegraphics[width=0.35\linewidth]{araug/04_00}} \hspace{2ex}
\subfloat[1:2]{\includegraphics[width=0.12\linewidth]{araug/04_05}}
\\[-0.5ex]
\subfloat[18:5]{\includegraphics[width=0.5\linewidth]{araug/04_01}}
\\[-0.5ex]
\subfloat[5:3]{\includegraphics[width=0.5\linewidth]{araug/04_03}} 

\mycaption{\acs{araug}}{%
Sample training images generated using the proposed augmentation strategy. 
This augmentation prevents overfitting to image shapes and increases the diversity of images seen by the network.
}




==> Figures/augs.tex <==
% Aspect ratio augmentation.

\def\w{0.25}



\includegraphics[width=\w\linewidth]{augs/target}
\includegraphics[width=\w\linewidth]{augs/pred_target}

\vspace{0.7ex}

\foreach \num in {00,05,10,17}{%
    \includegraphics[width=\w\linewidth]{augs/rand_\num}%
}
\\[-0.5ex]
\foreach \num in {00,05,10,17}{%
    \includegraphics[width=\w\linewidth]{augs/pred_rand_\num}%
}

\vspace{0.7ex}

\foreach \num in {04,10,13,16}{%
    \includegraphics[width=\w\linewidth]{augs/cutout_\num}%
}
\\[-0.5ex]
\foreach \num in {04,10,13,16}{%
    \includegraphics[width=\w\linewidth]{augs/pred_cutout_\num}%
}


% \foreach \num in {02,04,09,10,13,16}{%
% \foreach \num in {00,01,05,08,10,17}{%

% \includegraphics[width=\w\linewidth]{augs/target}
% \foreach \num in {04,10,13,16}{%
%     \includegraphics[width=\w\linewidth]{augs/cutout_\num}%
% }
% \\[-0.5ex]
% \includegraphics[width=\w\linewidth]{augs/pred_target}
% \foreach \num in {04,10,13,16}{%
%     \includegraphics[width=\w\linewidth]{augs/pred_cutout_\num}%
% }
% \\[0.5ex]
% \includegraphics[width=\w\linewidth]{augs/target}
% \foreach \num in {00,05,10,17}{%
%     \includegraphics[width=\w\linewidth]{augs/rand_\num}%
% }
% \\[-0.5ex]
% \includegraphics[width=\w\linewidth]{augs/pred_target}
% \foreach \num in {00,05,10,17}{%
%     \includegraphics[width=\w\linewidth]{augs/pred_rand_\num}%
% }


\mycaption{Photometric Augmentations}{%
Sample augmentations produced by RandAugment~\cite{Cubuk2020} and CutOut~\cite{Devries2017}.
The resulting model is highly robust to changing illumination conditions and is capable of filling in masked regions from the surrounding context. 
This can be seen in large regions of the ground-plane and connecting the tree trunk.
}


==> Figures/datasets.tex <==
% SlowTV sample images.

\def\w{0.17}

\foreach \img in {natural,driving,underwater,ctv}{%
    \foreach \num in {0,1,2,3,4,5}{%
        \includegraphics[width=\w\linewidth]{datasets/\img_\num}%
    }%
    \\[-0.3ex]%
}%


\mycaption{\acl{stv} \& \acl{ctv}}{%
Sample images from the proposed datasets, featuring diverse scenes for hiking, driving, scuba diving and real estate. 
The datasets consist of 45 videos curated from YouTube with a total of 2M training frames. 
Diversifying the training data allows our \acl{ssmde} models to generalize to unseen datasets.
We make the list of URLs and tools to process publicly available.
}


==> Figures/distort.tex <==
% Example of distorting image to training size.

\subfloat[Image]{\includegraphics[width=0.49\linewidth]{distort/104_img}} \hfill
\subfloat[Ground-truth]{\includegraphics[width=0.49\linewidth]{distort/104_depth}} 
\\[-2ex]
\subfloat[Base ($\delta_{.25} = 61.82\%$)]{\includegraphics[width=0.49\linewidth]{distort/104_pred1}}  \hfill
\subfloat[Distorted ($\delta_{.25} = \best{71.12\%}$)]{\includegraphics[width=0.49\linewidth]{distort/104_pred2}} 


\mycaption{Image Shape Overfitting}{%
The same model can produce significantly different results with different resolution images. 
Distorting the image to the original training resolution can improve performance, despite introducing stretching/squashing artifacts. 
Note, for instance, the improved boundary sharpness in \textbf{(d)}.
}


==> Figures/intro.tex <==
% Intro teaser. Note that this is a banner figure. 

\captionsetup{type=figure}

\subfloat{\includegraphics[width=0.2\linewidth]{intro/06_00_img}}%
\subfloat{\includegraphics[width=0.2\linewidth]{intro/06_01_depth}}%
\subfloat{\includegraphics[width=0.2\linewidth]{intro/06_03_kbr++}}%
\subfloat{\includegraphics[width=0.2\linewidth]{intro/06_03_kbr}}%
\subfloat{\includegraphics[width=0.2\linewidth]{intro/06_02_base}}%
\\[-2.5ex]
\setcounter{subfigure}{0}% Reset subfigure counter
\subfloat[\textbf{Image}]{\includegraphics[width=0.2\linewidth]{intro/09_00_img}}%
\subfloat[\textbf{Ground-truth}]{\includegraphics[width=0.2\linewidth]{intro/09_01_depth}}%
\subfloat[\textbf{\acs{kbr++}(Ours)}]{\includegraphics[width=0.2\linewidth]{intro/09_03_kbr++}}%
\subfloat[\textbf{\acs{kbr} (Ours)}]{\includegraphics[width=0.2\linewidth]{intro/09_03_kbr}}%
\subfloat[\textbf{Baseline~\cite{Spencer2022}}]{\includegraphics[width=0.2\linewidth]{intro/09_02_base}}%


\mycaption{Zero-shot generalization}{%
Our \acs{ssmde} models generalize to a wide range of complex environments. 
These models are trained on the novel large-scale \acl{stv} and \acl{ctv} datasets and can match or even surpass supervised \acs{sota}.
}


==> Figures/mapfree.tex <==

\tiny
\def\w{0.16}


\def\datas{
    img/Image
    ,depth/DPT-Kitti\textcolor{white}{++}
    ,kbr_base_042/KBR\textcolor{white}{++}
    ,kbr++_beitl_195/KBR++
}

\def\nums{
    0263%
    ,4990%
    ,7831%
    ,8292%
    ,14680%
    ,33435%
}


\foreach \method/\label in \datas{%
    \rotatebox{90}{\textbf{\label}}%
    \foreach \num in \nums{% 
        \includegraphics[width=\w\linewidth]{mapfree/mapfree_\num_\method}\hfill%
    } \\
}


\mycaption{MapFreeReloc~\cite{Arnold2022} Predictions}{%
Our models are capable of adapting to the challenging portrait images of the MapFreeReloc benchmark, allowing us to outperform other (self-)supervised methods. 
Our predictions are sharper and more detailed that those provided by the baseline, which requires a large collection of ground-truth annotations during training.
}

==> Figures/mdec.tex <==
% MDEC-2 validation leaderoard

\subfloat[Val]{\includegraphics[width=1\linewidth]{Images/mdec2_val.png}}

\subfloat[Test]{\includegraphics[width=1\linewidth]{Images/mdec2_test.png}}

\mycaption{MDEC-2~\cite{Spencer2023b}}{%
Our submission (\emph{jspenmar2}) was top of the leaderboard in pointcloud F-Score reconstruction. 
The challenge evaluated zero-shot performance on \acl{syns} for both supervised and self-supervised approaches.
}


==> Figures/slowtv.tex <==
% SlowTV sample images.

\def\w{0.166}

\foreach \img in {natural,driving,underwater}{%
    \foreach \num in {00, 01}{%
        \includegraphics[width=\w\linewidth]{slowtv/\num_\img}%
    }%
}%
\\[-0.3ex]
\foreach \img in {natural,driving,underwater}{%
    \foreach \num in {02, 03}{%
        \includegraphics[width=\w\linewidth]{slowtv/\num_\img}%
    }%
}%


\mycaption{\acl{stv}}{%
Sample images from the proposed dataset, featuring diverse scenes for hiking, driving and scuba diving. 
The dataset consists of 40 videos curated from YouTube, totalling to 1.7M frames. 
Diversifying the training data allows our \acl{ssmde} models to generalize to unseen datasets.
}


==> Figures/supp_araug.tex <==
% Supplementary aspect ratio augmentation visualizations.

% \subfloat[Original (16:9)]{\includegraphics[width=0.345\linewidth]{araug/00_00}}\hfill
% \subfloat[4:5]{\includegraphics[width=.145\linewidth]{araug/00_04}}\hfill
% \subfloat[Original (16:9)]{\includegraphics[width=0.245\linewidth]{araug/01_00}}\hfill
% \subfloat[5:3]{\includegraphics[width=.245\linewidth]{araug/01_01}}
% \\[-0.5ex]
% \subfloat[Original (16:9)]{\includegraphics[width=0.245\linewidth]{araug/05_00}}\hfill
% \subfloat[2:1]{\includegraphics[width=.245\linewidth]{araug/05_05}}\hfill
% \subfloat[Original (16:9)]{\includegraphics[width=0.295\linewidth]{araug/09_00}}\hfill
% \subfloat[1:1]{\includegraphics[width=.195\linewidth]{araug/09_02}}
\vspace{-0.25cm}

\subfloat[Original (16:9)]{\includegraphics[width=0.69\linewidth]{araug/00_00}}\hfill
\subfloat[4:5]{\includegraphics[width=.29\linewidth]{araug/00_04}}\hfill
\subfloat[Original (16:9)]{\includegraphics[width=0.49\linewidth]{araug/01_00}}\hfill
\subfloat[5:3]{\includegraphics[width=.49\linewidth]{araug/01_01}}
\\[-0.5ex]
\subfloat[Original (16:9)]{\includegraphics[width=0.49\linewidth]{araug/05_00}}\hfill
\subfloat[2:1]{\includegraphics[width=.49\linewidth]{araug/05_05}}\hfill
\subfloat[Original (16:9)]{\includegraphics[width=0.59\linewidth]{araug/09_00}}\hfill
\subfloat[1:1]{\includegraphics[width=.39\linewidth]{araug/09_02}}


\mycaption{\acs{araug}}{%
Additional augmentations used to diversify the variety of image shapes and object scales seen by the network.
}
\vspace{-0.5cm}


==> Figures/supp_slowtv.tex <==
% Supplementary SlowTV images (one per video). 

\newcommand{\numrows}{8}
\newcommand{\numcols}{5}
\def\w{.2}

\newcounter{i}
\newcounter{j}
\newcounter{ij}

% Zero-padding for sequence number
\renewcommand{\theij}{%
  \ifnum\value{ij}<10 0\fi
  \ifnum\value{ij}<100 000\fi
  \the\value{ij}%
}

\forloop{i}{0}{\value{i}<\numrows}{%
    \forloop{j}{0}{\value{j}<\numcols}{%
        \setcounter{ij}{\value{i}*\numcols + \value{j}}%
        \includegraphics[width=\w\linewidth]{slowtv_all/\theij}%
    } \\[-0.3ex]

}
\mycaption{\acl{stv} Dataset}{%
We show one frame per video from the proposed \acl{stv}. 
The dataset contains a diverse set of environments in a range of environmental conditions. 
The final dataset has a total of 1.7M images, with 1.15M natural, 400k driving and 180k underwater.
}


==> Figures/supp_slowtv_map.tex <==
% Supplementary SlowTV video locations on world map.

\includegraphics[width=0.8\linewidth]{slowtv_map}

\mycaption{\acl{stv} Map}{%
We show the map location for each sequence in \acl{stv}.
The distribution of locations ensures that the training data is highly diverse.
\textcolor{ForestGreen}{\textbf{Green}}=Natural, \textcolor{red}{\textbf{Red}}=Driving, \textcolor{blue}{\textbf{Blue}}=Underwater.
}


==> Figures/viz_fail.tex <==
% Zero-shot depth estimation failure cases.

\tiny

\def\w{0.103}

\def\datas{
    img/Image
    ,depth/GT
}

\def\selfsup{
    % ,garg/Garg~\cite{Garg2016}
    % ,monodepth2_MS/Monodepth2~\cite{Godard2019}
    hrdepth_MS/HR-Depth
    ,base/KBR
    ,kbr++_beitl_195/KBR++
}

\def\sup{
    MiDaS/MiDaS
    % ,DPT_Large/DPT-ViT~\cite{Ranftl2021}
    ,DPT_BEiT_L_512/DPT-BEiT
    ,newcrfs/NeWCRFs
}

\def\nums{
    viz_base/kitti_eigen_benchmark_0234%
    ,viz_zero_out/syns_test_0026%
    ,viz_zero_out/sintel_0086%
    ,viz_base/mc_0513%
    ,viz_zero_out/ddad_0521%
    ,viz_zero_out/diode_outdoor_0336%
    ,viz_zero_in/diode_indoors_0110%
    ,viz_zero_in/nyud_0055%
    ,viz_zero_in/tum_0668%
}

\def\ds{
    Kitti
    ,SYNS
    ,Sintel
    ,Mannequin
    ,DDAD
    ,Diode
    ,Diode
    ,NYUD
    ,TUM
}

\def\divider{\textcolor{black}{\hdashrule[2mm][x]{\linewidth}{\heavyrulewidth}{2pt}}}


\noindent
\rotatebox{90}{\color{white}{\textbf{Tmp}}}
\foreach \d in \ds{\makebox[\w\linewidth][c]{\textbf{\d}}\hfill}

\foreach \method/\label in \datas{%
    \rotatebox{90}{\textbf{\label}}
    \foreach \num in \nums{% 
        \includegraphics[width=\w\linewidth]{\num_\method}\hfill%
    } \\
}

\divider

\foreach \method/\label in \selfsup{%
    \rotatebox{90}{\textbf{\label}}
    \foreach \num in \nums{% 
        \includegraphics[width=\w\linewidth]{\num_\method}\hfill%
    } \\
}

\divider

\foreach \method/\label in \sup{%
    \rotatebox{90}{\textbf{\label}}
    \foreach \num in \nums{% 
        \includegraphics[width=\w\linewidth]{\num_\method}\hfill%
    } \\
}

\mycaption{Failure Cases}{%
The proposed model occasionally produces holes of infinite depth or texture-copy artifacts. 
However, complex regions such as foliage or object boundaries tend to be challenging for all approaches. 
Finally, the upright prior in training data makes the model sensitive to strong rotations. 
\emph{Middle=Self-Supervised -- Bottom=Supervised.}
}


==> Figures/viz_motion.tex <==
% Zero-shot depth estimation failure cases.

\tiny
\def\w{0.24}

\def\datas{
    img/Image
    ,depth/GT
}

\def\models{
    % ,garg/Garg~\cite{Garg2016}
    % ,monodepth2_MS/Monodepth2~\cite{Godard2019}
    % hrdepth_MS/HR-Depth
    % ,base/Ours
    full_no_md2_042/Baseline
    ,full_md2_042/Monodepth2
}

\def\nums{
    viz_motion/kitti_eigen_benchmark_0408%
    ,viz_motion/sintel_0570%
    ,viz_motion/ddad_0973%
    ,viz_motion/tum_1064%
}


\foreach \method/\label in \datas{%
    \rotatebox{90}{\textbf{\label}}
    \foreach \num in \nums{% 
        \includegraphics[width=\w\linewidth]{\num_\method}\hfill%
    } \\
}

\foreach \method/\label in \models{%
    \rotatebox{90}{\textbf{\label}}
    \foreach \num in \nums{% 
        \includegraphics[width=\w\linewidth]{\num_\method}\hfill%
    } \\
}

\mycaption{Dynamic Object Robustness}{%
Incorporating the contributions from Monodepth2~\cite{Godard2019} mitigates artifacts from dynamic objects and improves the sharpness of depth discontinuities. 
This is achieved in a cost-effective manner, without requiring complex consistency losses or additional annotations. 
}


==> Figures/viz_zero.tex <==
% Zero-shot depth estimation.

\def\w{0.105}
\tiny

\scriptsize

% \def\methods{
%     img/Image
%     ,depth/GT
%     % ,learn_K/Ours
%     ,base/Ours
%     % ,garg/Garg~\cite{Garg2016}
%     % ,monodepth2_MS/Monodepth2~\cite{Godard2019}
%     ,hrdepth_MS/HR-Depth~\cite{Lyu2021}
%     ,MiDaS/MiDaS~\cite{Ranftl2020}
%     % ,DPT_Large/DPT-ViT~\cite{Ranftl2021}
%     ,DPT_BEiT_L_512/DPT-BEiT~\cite{Ranftl2021}
%     ,newcrfs/NeWCRFs~\cite{Weihao2022}
% }

% \def\methods{
%     img/Image
%     ,depth/GT
%     % ,learn_K/Ours
%     ,base/Ours
%     % ,garg/Garg~\cite{Garg2016}
%     % ,monodepth2_MS/Monodepth2~\cite{Godard2019}
%     ,hrdepth_MS/HR-Depth
%     ,MiDaS/MiDaS
%     % ,DPT_Large/DPT-ViT~\cite{Ranftl2021}
%     ,DPT_BEiT_L_512/DPT-BEiT
%     ,newcrfs/NeWCRFs
% }

\tiny

\def\datas{
    img/Image
    ,depth/GT
}

\def\selfsup{
    % ,garg/Garg~\cite{Garg2016}
    % ,monodepth2_MS/Monodepth2~\cite{Godard2019}
    hrdepth_MS/HR-Depth
    ,base/KBR
    ,kbr++_beitl_195/KBR++
}

\def\sup{
    MiDaS/MiDaS
    % ,DPT_Large/DPT-ViT~\cite{Ranftl2021}
    ,DPT_BEiT_L_512/DPT-BEiT
    ,newcrfs/NeWCRFs
}


\def\nums{
    viz_base/kitti_eigen_benchmark_0072%
    ,viz_zero_out/syns_test_0374%
    ,viz_zero_out/sintel_0411%
    ,viz_base/mc_0938%
    ,viz_zero_out/ddad_0737%
    ,viz_zero_out/diode_outdoor_0030%
    ,viz_zero_in/diode_indoors_0139%
    ,viz_zero_in/nyud_0247%
    ,viz_zero_in/tum_0246%
}

\def\ds{
    Kitti
    ,SYNS
    ,Sintel
    ,Mannequin
    ,DDAD
    ,DIODE
    ,DIODE
    ,NYUD-v2
    ,TUM
}

\def\divider{\textcolor{black}{\hdashrule[1mm][x]{\linewidth}{\heavyrulewidth}{2pt}}}

\noindent
\rotatebox{90}{\color{white}{\textbf{Tmp}}}
\foreach \d in \ds{\makebox[\w\linewidth][c]{\textbf{\d}}\hfill}

\foreach \method/\label in \datas{%
    \rotatebox{90}{\textbf{\label}}
    \foreach \num in \nums{% 
        \includegraphics[width=\w\linewidth]{\num_\method}\hfill%
    } \\
}

\divider

\foreach \method/\label in \selfsup{%
    \rotatebox{90}{\textbf{\label}}
    \foreach \num in \nums{% 
        \includegraphics[width=\w\linewidth]{\num_\method}\hfill%
    } \\
}

\divider

\foreach \method/\label in \sup{%
    \rotatebox{90}{\textbf{\label}}
    \foreach \num in \nums{% 
        \includegraphics[width=\w\linewidth]{\num_\method}\hfill%
    } \\
}

\mycaption{Zero-shot \acl{ssmde}}{%
The proposed \acs{kbr} models generalize to a wide range of scene types, greatly improving upon the \ac{ssl} baselines. 
The contributions from this paper further improve robustness to indoor scenes and the accuracy at thin structures. 
\emph{Middle=Self-Supervised -- Bottom=Supervised.}
}


==> Tables/datasets.tex <==
% Summary of training & eval datasets.

% \tiny

\mycaption{Datasets Comparison}{%
The top half shows commonly used \acl{ssmde} training datasets.
% Existing datasets focus exclusively on urban automotive data. 
\acl{stv} and \acl{ctv} greatly diversify the training environments and scale to much larger data quantities.
The bottom half summarizes the testing datasets used in our \emph{zero-shot generalization} evaluation.
}

\begin{tabular}{lccccccccc}
\toprule
                                        &  Urban & Natural &  Scuba & Indoor &       Depth &    Acc & Density &         \#Img \\
\midrule      
Kitti~\cite{Geiger2013,Uhrig2018}\mydag & \cmark &  \xmark & \xmark & \xmark & \acs{lidar} &   High &     Low &           71k \\
\acl{ddad}~\cite{Guizilini2020}         & \cmark &  \xmark & \xmark & \xmark & \acs{lidar} &    Mid &     Low &           76k \\
CityScapes~\cite{Cordts2016}            & \cmark &  \xmark & \xmark & \xmark &      Stereo &    Low &     Mid &           88k \\
Mannequin~\cite{Li2020}\mydag           & \cmark &  \xmark & \xmark & \cmark &    \ac{sfm} &    Mid &     Mid &          115k \\
\textbf{\acl{stv} (Ours)}\mydag         & \cmark &  \cmark & \cmark & \xmark &      \xmark & \xmark &  \xmark & \textbf{1.7M} \\
\textbf{\acl{ctv} (Ours)}\mydag         & \cmark &  \xmark & \xmark & \cmark &      \xmark & \xmark &  \xmark & \textbf{330k} \\
\midrule                             
Kitti~\cite{Geiger2013,Uhrig2018}       & \cmark &  \xmark & \xmark & \xmark & \acs{lidar} &   High &     Low &           652 \\
\acl{ddad}~\cite{Guizilini2020}         & \cmark &  \xmark & \xmark & \xmark & \acs{lidar} &    Mid &     Low &            1k \\
\acl{sintel}~\cite{Butler2012}          & \xmark &  \cmark & \xmark & \xmark &       Synth &   High &    High &          1064 \\
\acl{syns}~\cite{Adams2016,Spencer2022} & \cmark &  \cmark & \xmark & \cmark & \acs{lidar} &   High &    High &           775 \\
\acs{dii}~\cite{Vasiljevic2019}         & \cmark &  \xmark & \xmark & \cmark & \acs{lidar} &   High &    High &           771 \\
Mannequin~\cite{Li2020}                 & \cmark &  \xmark & \xmark & \cmark &    \ac{sfm} &    Mid &     Mid &            1k \\
\acl{nyud}~\cite{Silberman2012}         & \xmark &  \xmark & \xmark & \cmark &      Kinect &    Mid &    High &           654 \\
\acl{tum}~\cite{Sturm2012}              & \xmark &  \xmark & \xmark & \cmark &      Kinect &    Mid &    High &          2.5k \\
\bottomrule
\end{tabular}

\centering
\emph{%
\mydag Datasets used to train our networks.
}


==> Tables/mapfree.tex <==
% MapFreeReloc benchmark results.
\addtolength{\tabcolsep}{-0.1em}

\mycaption{Map-free Relocalization~\cite{Arnold2022}}{%
The feature-matching MapFreeReloc baselines~\cite{Arnold2022} can be improved with our novel \acs{ssmde} models. 
These results are zero-shot, without finetuning on the target dataset (which consists of portrait images).
The improved variants from this paper (\acs{kbr++}) perform on-par with \acl{dpt-beit} and outperform every other (self-)supervised approach. 
}

\begin{tabular}{@{}lllllllllll@{}}
\toprule
                                &       & \multicolumn{2}{c}{Multi-task} &                                   \multicolumn{4}{c}{Pose} &                       \multicolumn{3}{c}{VCRE} \\
                                          \cmidrule(lr){3-4}                                          \cmidrule(lr){5-8}                               \cmidrule(lr){9-11}
                                & Train &    \acs{rank}\down &        \acs{relimp}\up &   Trans\down &      Rot\down &         P\up &        AUC\up &     Error\down &          P\up &        AUC\up \\
\midrule  
         Garg~\cite{Garg2016}   &     S &        10.50 &       -21.84 &         2.96 &         52.57 &          5.43 &         17.15 &         188.20 &         24.84 &         51.61 \\ 
 Monodepth2~\cite{Godard2017}   &    MS &        11.25 &       -22.32 &         2.95 &         52.92 &          5.50 &         17.22 &         189.67 &         24.38 &         50.63 \\ 
      DiffNet~\cite{Zhou2021}   &    MS &        10.88 &       -21.70 &         2.97 &         53.19 &          5.65 &         17.71 &         188.80 &         24.78 &         51.24 \\ 
      HR-Depth~\cite{Lyu2021}   &    MS &         9.38 &       -21.07 &         2.94 &         52.95 &          5.67 &         17.95 &         187.83 &         25.06 &         51.52 \\ 
\midrule
    \textbf{\acs{kbr} (Ours)}   &     M &         4.50 &         0.00 & \nbest{2.63} & \nbest{49.01} & \nbest{11.54} & \nbest{32.02} & \nbest{181.21} & \nbest{29.96} & \nbest{58.89} \\ 
    \textbf{\acs{kbr++} (Ours)} &     M & \nbest{2.00} & \nbest{4.86} &  \best{2.58} &  \best{46.22} &  \best{12.50} &  \best{33.76} &  \best{178.26} &  \best{31.93} &  \best{61.48} \\ 
\midrule
\midrule
      MiDaS~\cite{Ranftl2020}   &     D &         4.00 &         0.35 &         2.60 &         46.92 & \nbest{11.39} &         30.44 & \nbest{180.64} &         30.45 &         59.72 \\ 
    DPT-ViT~\cite{Ranftl2021}   &     D &         3.38 &         1.09 & \nbest{2.56} & \nbest{45.62} &         11.27 & \nbest{30.92} &         181.34 & \nbest{30.60} & \nbest{60.03} \\ 
   DPT-BEiT~\cite{Ranftl2021}   &     D &  \best{1.75} &  \best{5.32} &  \best{2.49} &  \best{44.99} &  \best{12.56} &  \best{32.48} &         181.67 &  \best{32.46} &  \best{62.03} \\ 
    NeWCRFs~\cite{Weihao2022}   &     D &         8.00 &       -16.98 &         2.89 &         51.92 &          6.69 &         20.77 &         184.63 &         25.89 &         52.93 \\ 
\midrule   
   DPT-NYUD~\cite{Arnold2022}   &  D+FT &         6.50 &        -6.61 &         2.67 &         47.66 &          9.17 &         26.46 &         184.53 &         28.68 &         56.87 \\ 
  DPT-Kitti~\cite{Arnold2022}   &  D+FT &         5.88 &        -3.05 &         2.66 &         49.21 &         10.86 &         29.99 &  \best{178.49} &         28.37 &         56.86 \\ 
\bottomrule
\end{tabular}

\centering
\emph{%
\textbf{Trans}=meters, \textbf{Rot}=deg, \textbf{VCRE}=px, \textbf{Precision}=\%, \textbf{AUC}=\%.
}


==> Tables/reb_dynamic.tex <==

\def\mc{\multicolumn}
\addtolength{\tabcolsep}{0.2em}
\footnotesize

\mycaption{Dynamic Object Results}{%
The losses from Monodepth2 improve performance in datasets with dynamic objects, despite not explicitly modelling their motion.
This ablation was conducted using ConvNeXt-Tiny and a small subset of all datasets.
}

\begin{tabular}{@{}llllllllll@{}}
\toprule
                 & \mc{2}{c}{\textbf{\acs{keb}}} & \mc{2}{c}{\textbf{\acs{ddad}}} & \mc{2}{c}{\textbf{\acs{sintel}}} \\ 
                              \cmidrule(lr){2-3}               \cmidrule(lr){4-5}                 \cmidrule(lr){6-7}
                 &     Rel\down & F\up &      Rel\down &          F\up &      Rel\down & F\up \\ 
\midrule
Baseline         & \nbest{9.00} & \nbest{53.50} & \nbest{23.57} & \nbest{11.13} & \nbest{35.33} & \nbest{38.15} \\ 
MinRec+Automask  &  \best{6.50} &  \best{55.62} &  \best{18.49} &  \best{11.64} &  \best{34.97} &  \best{38.83} \\ 
\bottomrule
\end{tabular}




% \begin{tabular}{@{}llllllllll@{}}
% \toprule
%                             &           \multicolumn{3}{c}{\textbf{\acs{keb}}} &             \multicolumn{3}{c}{\textbf{\acs{ddad}}} & \multicolumn{3}{c}{\textbf{\acs{sintel}}} \\ 
%                                                             \cmidrule(lr){2-4}                                  \cmidrule(lr){5-7}                                \cmidrule(lr){8-10}
%                             &     Rel\down & \acs{d25}\up &          F\up &      Rel\down & \acs{d25}\up &          F\up &      Rel\down & \acs{d25}\up &          F\up \\ 
% \midrule
% Default &  \best{6.99} & \nbest{55.80} &      \best{94.16} & \nbest{12.27} &  \best{21.09} &      \best{86.14} & \nbest{33.23} & \nbest{40.20} &     \nbest{57.35} \\ 
% MinRec+Automask & \nbest{7.01} &  \best{55.92} &     \nbest{94.06} &  \best{12.18} & \nbest{20.72} &     \nbest{86.07} &  \best{33.00} &  \best{41.59} &      \best{59.40} \\ 
% \bottomrule
% \end{tabular}

==> Tables/reb_kitti.tex <==

\def\mc{\multicolumn}
\addtolength{\tabcolsep}{0.2em}
\small

% \mycaption{\acl{keb} Results}{%
% Performance when training on Kitti with/without camera intrinsics learning.
% }

\mycaption{\acl{kez} Results}{%
Learning \acs{Cam} gives comparable performance even when training only on Kitti.
% Learning \acs{Cam} improves performance even when training only on Kitti.
}


% \begin{tabular}{@{}lllllll@{}}
% \toprule
%                 & \mc{2}{c}{\textbf{\acs{keb}}} & \mc{2}{c}{\textbf{\acs{mc}}} & \mc{2}{c}{\textbf{\acs{syns}}} \\ 
%                              \cmidrule(lr){2-3}             \cmidrule(lr){4-5}               \cmidrule(lr){6-7}
%                 &               Rel\down & F\up &              Rel\down & F\up &                Rel\down & F\up \\ 
% \midrule
% Baseline        &  0 & 0 &  0 &  0 & 0 & 0 \\ 
% Learn \acs{Cam} &  0 & 0 &  0 &  0 & 0 & 0 \\  
% \bottomrule
% \end{tabular}

% \begin{tabular}{@{}llll@{}}
% \toprule
%                 &     Rel\down &          F\up & \acs{d25}\up \\ 
% \midrule
% Baseline        &  \best{7.19} & \nbest{54.70} &      \best{93.56} \\ 
% Learn \acs{Cam} & \nbest{7.32} &  \best{54.87} &     \nbest{93.17} \\ 
% \bottomrule
% \end{tabular}


\begin{tabular}{@{}llll@{}}
\toprule
                &     Rel\down &          F\up & \acs{d25}\up \\ 
\midrule
Baseline        & \nbest{5.69} &  \best{60.88} &     \nbest{95.89} \\ 
Learn \acs{Cam} &  \best{5.68} & \nbest{60.81} &      \best{95.90} \\ 
\bottomrule
\end{tabular}

==> Tables/res.tex <==
% Results on all datasets.

\addtolength{\tabcolsep}{-0.1em}
\def\mc{\multicolumn}

\mycaption{Results}{%
\emph{Outdoor} and \emph{Indoor} represent zero-shot evaluations. 
We outperform all \acl{ssmde} baselines~\cite{Spencer2022} (top block).
Our original model (\acs{kbr}) performs on par with the supervised \ac{sota}, while the updated model from this paper (\acs{kbr++}) outperforms every model except \acs{dpt-beit}~\cite{Ranftl2021}. 
Our models do not required ground-truth annotations for training and instead leverage large-scale YouTube data.
}

\begin{adjustbox}{center}

\begin{tabular}{@{}llllllllllllllllllllll@{}}
\toprule
                             &       &&& \mc{4}{c}{\bf{In-Distribution}}                                         & \mc{8}{c}{\bf{Outdoor}}                                                                                                       & \mc{6}{c}{\bf{Indoor}}                                                                            \\
                                       \cmidrule(lr){5-8}                                                        \cmidrule(lr){9-16}                                                                                                             \cmidrule(lr){17-22}
                             &       & \mc{2}{c}{\textbf{Multi-task}} & \mc{2}{c}{\bf\acs{keb}}            & \mc{2}{c}{\bf\acs{mc}}             & \mc{2}{c}{\bf\acs{ddad}}      & \mc{2}{c}{\bf\acs{dio}}       & \mc{2}{c}{\bf\acs{sintel}}    & \mc{2}{c}{\bf\acs{syns}}      & \mc{2}{c}{\bf\acs{dii}}       & \mc{2}{c}{\bf\acl{nyud}}          & \mc{2}{c}{\bf\acs{tum}}       \\  
                                       \cmidrule(lr){3-4}                   \cmidrule(lr){5-6}                   \cmidrule(lr){7-8}              \cmidrule(lr){9-10}             \cmidrule(lr){11-12}            \cmidrule(lr){13-14}            \cmidrule(lr){15-16}            \cmidrule(lr){17-18}                \cmidrule(lr){19-20}  \cmidrule(lr){21-22}
                             & Train &    \acs{rank}\down &        \acs{relimp}\up &        Rel\down &             F\up &         Rel\down &            F\up &      Rel\down &          F\up &      Rel\down &  \acs{d25}\up &      Rel\down &          F\up &      Rel\down &          F\up &      Rel\down &  \acs{d25}\up &       Rel\down &     \acs{d25}\up &      Rel\down &  \acs{d25}\up \\
\midrule
Garg~\cite{Garg2016}         & S     &         7.58 &       -38.52 &    \zs     7.65 &   \zs      53.28 &         27.63 &          9.08 &         26.93 &          7.80 &         39.60 &             44.15 &         39.41 &         31.93 &         26.05 &         15.17 &         19.18 &             70.54 &         22.49 &             59.60 &         23.53 &             62.82 \\
Monodepth2~\cite{Godard2019} & MS    &         7.74 &       -38.34 &    \zs     7.90 &   \zs      50.50 &         27.44 &          7.97 &         24.31 &          8.25 &         39.53 &             44.71 &         40.09 &         29.49 &         25.31 &         14.83 &         19.40 &             70.42 &         22.41 &             60.09 &         23.50 &             62.36 \\
DiffNet~\cite{Zhou2021}      & MS    &         7.05 &       -36.84 &    \zs     7.98 &   \zs      49.60 &         27.46 &          7.76 &         23.03 &          9.43 &         38.87 &             46.14 &         39.93 &         28.77 &         25.09 &         14.64 &         19.11 &             70.94 &         21.82 &             61.30 &         23.21 &             63.08 \\
HR-Depth~\cite{Lyu2021}      & MS    &         5.95 &       -35.16 &    \zs     7.70 &   \zs      51.49 &         27.01 &          8.39 &         23.13 &          9.94 &         39.09 &             45.60 &         38.82 &         30.90 &         25.07 &         15.48 &         18.93 &             71.19 &         21.74 &             61.18 &         23.18 &             63.50 \\
\midrule
\textbf{\acs{kbr} (Ours)~\cite{Spencer2023c}}      & M     &         3.37 &         0.00 & \zs\nbest{6.84} & \zs\nbest{56.17} & \zs\nbest{14.39} & \zs\nbest{17.67} &  \best{12.63} &  \best{20.21} & \nbest{33.49} &     \nbest{57.08} & \nbest{33.34} & \nbest{40.81} & \nbest{22.40} & \nbest{18.50} & \nbest{14.91} &     \nbest{80.77} & \nbest{11.59} &     \nbest{87.23} & \nbest{15.02} &     \nbest{80.86} \\
\textbf{\acs{kbr++} (Ours)}    & M     & \nbest{2.95} & \nbest{4.58} &  \zs\best{6.77} &  \zs\best{56.57} &  \zs\best{12.95} &  \zs\best{20.08} & \nbest{13.10} & \nbest{17.87} &  \best{32.81} &      \best{57.77} &  \best{30.46} &  \best{41.89} &  \best{21.92} &  \best{18.79} &  \best{14.26} &      \best{82.94} &   \best{9.24} &      \best{91.85} &  \best{12.71} &      \best{85.86} \\
\midrule
\midrule
MiDaS~\cite{Ranftl2020}      & D     &         5.68 &       -11.84 &           13.71 &            33.44 &            16.96 &           12.62 &         16.00 &         15.41 &         32.72 &         59.04 &         30.95 &         39.55 &         26.94 &         14.69 &        10.71 &         88.42 &           10.48 &            89.59 &         14.43 &         82.35 \\
DPT-ViT~\cite{Ranftl2021}    & D     &         3.84 &        -1.74 &           10.98 &            40.56 &    \nbest{15.52} &           14.46 &         15.49 &         18.25 & \nbest{32.59} & \nbest{59.82} & \nbest{25.53} & \nbest{43.57} & \nbest{23.24} & \nbest{17.44} & \nbest{9.60} & \nbest{91.38} &           10.10 &            90.10 & \nbest{12.68} & \nbest{86.25} \\
DPT-BEiT~\cite{Ranftl2021}   & D     &  \best{2.11} & \best{11.12} & \zs\nbest{9.45} & \zs\nbest{44.22} &     \best{13.55} &    \best{16.58} & \nbest{10.70} & \nbest{22.63} &  \best{31.08} &  \best{61.51} &  \best{21.38} &  \best{46.46} &  \best{21.47} &  \best{17.73} &  \best{7.89} &  \best{93.34} & \zs \best{5.40} & \zs \best{96.54} &  \best{10.45} &  \best{89.68} \\
NeWCRFs~\cite{Weihao2022}    & D     &         3.84 &         1.03 &  \zs\best{5.23} &  \zs\best{59.20} &         18.20 & \nbest{15.17} &   \best{9.59} &  \best{23.02} &         37.01 &             49.66 &         39.25 &         32.43 &         24.28 &         16.76 &        14.05 &             84.95 & \zs\nbest{6.22} &     \zs\nbest{95.58} &         14.63 &             82.95 \\
\bottomrule
\end{tabular}
\end{adjustbox}

\emph{%
Highlighted cells are \emph{\textbf{NOT zero-shot}} results.
\textbf{S}=Stereo, \textbf{M}=Monocular, \textbf{D}=Ground-truth Depth.
}





% \addtolength{\tabcolsep}{0.2em}
% \def\mc{\multicolumn}
% 
% \mycaption{Results}{%
% \textit{Outdoor} and \textit{Indoor} represent zero-shot evaluations. 
% We outperform all \acl{ssmde} baselines~\cite{Spencer2022} (top block).
% In many cases, our model performs on par with supervised \ac{sota} (bottom block), without requiring ground-truth depth annotations for training. 
% }


% \begin{tabular}{@{}llllllllllllllllllll@{}}
% \toprule
%                              &       & \mc{4}{c}{\bf{In-Distribution}}                                         & \mc{8}{c}{\bf{Outdoor}}                                                                                                       & \mc{6}{c}{\bf{Indoor}}                                                                            \\
%                                        \cmidrule(lr){3-6}                                                        \cmidrule(lr){7-14}                                                                                                             \cmidrule(lr){15-20}
%                              &       & \mc{2}{c}{\bf\acs{keb}}            & \mc{2}{c}{\bf\acs{mc}}             & \mc{2}{c}{\bf\acs{ddad}}      & \mc{2}{c}{\bf\acs{dio}}       & \mc{2}{c}{\bf\acs{sintel}}    & \mc{2}{c}{\bf\acs{syns}}      & \mc{2}{c}{\bf\acs{dii}}       & \mc{2}{c}{\bf\acl{nyud}}          & \mc{2}{c}{\bf\acs{tum}}       \\  
%                                        \cmidrule(lr){3-4}                   \cmidrule(lr){5-6}                   \cmidrule(lr){7-8}              \cmidrule(lr){9-10}             \cmidrule(lr){11-12}            \cmidrule(lr){13-14}            \cmidrule(lr){15-16}            \cmidrule(lr){17-18}                \cmidrule(lr){19-20}
%                              & Train &        Rel\down &             F\up &         Rel\down &            F\up &      Rel\down &          F\up &      Rel\down &  \acs{d25}\up &      Rel\down &          F\up &      Rel\down &          F\up &      Rel\down &  \acs{d25}\up &       Rel\down &     \acs{d25}\up &      Rel\down &  \acs{d25}\up \\
% \midrule
% Garg~\cite{Garg2016}         & S     & \zs\nbest{7.65} & \zs\nbest{53.28} &            27.63 &    \nbest{9.08} &         26.93 &          7.80 &         39.60 &         44.15 &         39.41 & \nbest{31.93} &         26.05 &         15.17 &         19.18 &         70.54 &          22.49 &            59.60 &         23.53 &         62.82 \\ 
% Monodepth2~\cite{Godard2019} & MS    &         \zs7.90 &         \zs50.50 &            27.44 &            7.97 &         24.31 &          8.25 &         39.53 &         44.71 &         40.09 &         29.49 &         25.31 &         14.83 &         19.40 &         70.42 &          22.41 &            60.09 &         23.50 &         62.36 \\ 
% DiffNet~\cite{Zhou2021}      & MS    &         \zs7.98 &         \zs49.60 &            27.46 &            7.76 & \nbest{23.03} &          9.43 & \nbest{38.87} & \nbest{46.14} &         39.93 &         28.77 &         25.09 &         14.64 &         19.11 &         70.94 &          21.82 &    \nbest{61.30} &         23.21 &         63.08 \\ 
% HR-Depth~\cite{Lyu2021}      & MS    &         \zs7.70 &         \zs51.49 &    \nbest{27.01} &            8.39 &         23.13 &  \nbest{9.94} &         39.09 &         45.60 & \nbest{38.82} &         30.90 & \nbest{25.07} & \nbest{15.48} & \nbest{18.93} & \nbest{71.19} &  \nbest{21.74} &            61.18 & \nbest{23.18} & \nbest{63.50} \\ 
% \midrule
% % \textbf{\acs{kbr} (Ours)}    & M     &  \zs\best{6.86} &  \zs\best{59.22} &  \zs\best{15.94} & \zs\best{20.22} &  \best{13.91} &  \best{18.52} &  \best{34.53} &  \best{55.27} &  \best{33.32} &  \best{43.46} &  \best{23.46} &  \best{20.32} &  \best{16.10} &  \best{78.55} &   \best{13.76} &     \best{82.67} &  \best{17.70} &  \best{75.05} \\ 
% \textbf{\acs{kbr} (Ours)}    & M     &  \zs\best{6.84} &  \zs\best{56.17} &  \zs\best{14.39} & \zs\best{17.67} &  \best{12.63} & \best{20.21} &  \best{33.49} &      \best{57.08} &  \best{33.34} &  \best{40.81} &  \best{22.40} &  \best{18.50} &  \best{14.91} &      \best{80.77} &  \best{11.59} &      \best{87.23} &  \best{15.02} &      \best{80.86} \\

% \midrule
% \midrule
% MiDaS~\cite{Ranftl2020}      & D     &           13.71 &            33.44 &            16.96 &           12.62 &         16.00 &         15.41 &         32.72 &         59.04 &         30.95 &         39.55 &         26.94 &         14.69 &        10.71 &         88.42 &           10.48 &            89.59 &         14.43 &         82.35 \\
% DPT-ViT~\cite{Ranftl2021}    & D     &           10.98 &            40.56 &    \nbest{15.52} &           14.46 &         15.49 &         18.25 & \nbest{32.59} & \nbest{59.82} & \nbest{25.53} & \nbest{43.57} & \nbest{23.24} & \nbest{17.44} & \nbest{9.60} & \nbest{91.38} &           10.10 &            90.10 & \nbest{12.68} & \nbest{86.25} \\
% DPT-BEiT~\cite{Ranftl2021}   & D     & \zs\nbest{9.45} & \zs\nbest{44.22} &     \best{13.55} &    \best{16.58} & \nbest{10.70} & \nbest{22.63} &  \best{31.08} &  \best{61.51} &  \best{21.38} &  \best{46.46} &  \best{21.47} &  \best{17.73} &  \best{7.89} &  \best{93.34} & \zs \best{5.40} & \zs \best{96.54} &  \best{10.45} &  \best{89.68} \\
% NeWCRFs~\cite{Weihao2022}    & D     & \zs \best{5.23} & \zs \best{59.20} &            18.30 &   \nbest{15.07} &   \best{9.59} &  \best{23.02} &         34.24 &         55.54 &         39.26 &         32.43 &         24.28 &         16.76 &        14.05 &         84.95 & \zs\nbest{6.39} & \zs\nbest{95.53} &         14.63 &         82.95 \\
% \bottomrule
% \end{tabular}

% \emph{%
% Highlighted cells are \emph{\textbf{NOT zero-shot}} results.
% \textbf{S}=Stereo, \textbf{M}=Monocular, \textbf{D}=Ground-truth Depth.
% }

==> Tables/res_abl.tex <==
% Ablation experiments. 

% \addtolength{\tabcolsep}{-0.1em}

\footnotesize
\addtolength{\tabcolsep}{-0.1em}
\def\mc{\multicolumn}


\mycaption{Ablations}{%
We carry out ablations for each component in our framework.
From top to bottom: \acs{kbr}~\cite{Spencer2023c} contributions, network architecture, augmentations and datasets.
In each case, the proposed contributions improve the zero-shot generalization of our models.
}

\begin{adjustbox}{center}
\begin{tabular}{@{}lllllllllllllllllllll@{}}
\toprule
                             &&& \mc{4}{c}{\zs\bf{In-Distribution}}                                         & \mc{8}{c}{\bf{Outdoor}}                                                                                                       & \mc{6}{c}{\bf{Indoor}}                                                                            \\
                                       \cmidrule(lr){4-7}                                                        \cmidrule(lr){8-15}                                                                                                             \cmidrule(lr){16-21}
                             & \mc{2}{c}{\textbf{Multi-task}} & \mc{2}{c}{\bf\acs{keb}}            & \mc{2}{c}{\bf\acs{mc}}             & \mc{2}{c}{\bf\acs{ddad}}      & \mc{2}{c}{\bf\acs{dio}}       & \mc{2}{c}{\bf\acs{sintel}}    & \mc{2}{c}{\bf\acs{syns}}      & \mc{2}{c}{\bf\acs{dii}}       & \mc{2}{c}{\bf\acl{nyud}}          & \mc{2}{c}{\bf\acs{tum}}       \\  
                                       \cmidrule(lr){2-3}                   \cmidrule(lr){4-5}                   \cmidrule(lr){6-7}              \cmidrule(lr){8-9}             \cmidrule(lr){10-11}            \cmidrule(lr){12-13}            \cmidrule(lr){14-15}            \cmidrule(lr){16-17}                \cmidrule(lr){18-19}  \cmidrule(lr){20-21}
                             &    \acs{rank}\down &        \acs{relimp}\up &        Rel\down &             F\up &         Rel\down &            F\up &      Rel\down &          F\up &      Rel\down &  \acs{d25}\up &      Rel\down &          F\up &      Rel\down &          F\up &      Rel\down &  \acs{d25}\up &       Rel\down &     \acs{d25}\up &      Rel\down &  \acs{d25}\up \\
\midrule

\textbf{\acs{kbr}} &  \best{2.37} &   \best{0.00} & \nbest{6.84} &  \best{56.17} &         14.39 &         17.67 & \nbest{12.63} &  \best{20.21} & \nbest{33.49} &     \nbest{57.08} &         33.34 &         40.81 & \nbest{22.40} & \nbest{18.50} &         14.91 &             80.77 & \nbest{11.59} &     \nbest{87.23} & \nbest{15.02} &     \nbest{80.86} \\ 
         Fwd \acs{Pose} & \nbest{2.79} & \nbest{-0.64} &         7.27 &         54.61 &         14.36 &         17.52 &  \best{12.43} & \nbest{19.76} &         33.52 &             56.97 & \nbest{32.25} &         41.05 &  \best{22.32} &         18.45 & \nbest{14.89} &             80.54 &         11.68 &             87.14 &         15.50 &             80.29 \\ 
$\acs{offset} = \pm1$ &         3.16 &         -1.18 &  \best{6.79} & \nbest{55.92} &  \best{14.17} &  \best{17.92} &         13.66 &         19.18 &         33.75 &             56.56 &         32.30 & \nbest{41.14} &         23.05 &         17.90 &         15.00 &     \nbest{80.82} &         11.73 &             86.94 &         15.66 &             79.91 \\ 
            Fixed \acs{Cam} &         4.00 &         -2.76 &         7.09 &         55.19 &         14.95 &         17.11 &         14.30 &         18.15 &  \best{33.49} &      \best{57.10} &         33.39 &  \best{41.43} &         22.56 &  \best{18.67} &         15.41 &             79.98 &         12.06 &             86.14 &         15.75 &             80.07 \\ 
              No \ac{araug} &         3.53 &         -3.86 &         8.32 &         50.15 & \nbest{14.32} & \nbest{17.87} &         14.75 &         16.90 &         34.49 &             55.82 &         33.25 &         40.51 &         23.38 &         17.33 &  \best{14.58} &      \best{81.69} &  \best{11.24} &      \best{87.77} &  \best{14.61} &      \best{81.76} \\ 
        None &         5.16 &         -7.59 &         8.66 &         48.33 &         14.62 &         17.01 &         18.46 &         15.17 &         34.38 &             55.62 &  \best{31.88} &         40.27 &         23.32 &         17.97 &         15.15 &             80.30 &         11.88 &             86.35 &         15.55 &             79.81 \\ 
\midrule
       ConvNeXt-B &         3.47 &         0.00 &  \best{6.84} &  \best{56.17} &         14.39 &         17.67 &  \best{12.63} &  \best{20.21} &         33.49 &             57.08 &         33.34 &         40.81 & \nbest{22.40} & \nbest{18.50} &         14.91 &             80.77 &         11.59 &             87.23 &         15.02 &             80.86 \\ 
 ViT-B-384  &         4.68 &        -3.17 &         7.41 &         54.31 &         14.80 &         17.05 &         14.47 &         16.31 &         33.37 &             56.99 &         33.00 &         39.15 &         23.08 &         17.55 &         14.19 &             83.09 &         11.58 &             86.83 &         15.41 &             81.65 \\ 
 ViT-L-384 & \nbest{2.53} & \nbest{0.41} &         7.29 &         54.70 & \nbest{14.02} & \nbest{18.10} &         14.38 &         16.88 &         33.02 &             58.18 & \nbest{30.68} &  \best{42.01} &         22.51 &         17.83 & \nbest{13.72} &     \nbest{83.98} & \nbest{10.60} &     \nbest{88.96} & \nbest{14.07} &     \nbest{83.24} \\ 
BEiT-B-384 &         2.79 &         0.32 &         6.93 &         55.28 &         14.23 &         17.98 & \nbest{13.50} & \nbest{17.84} &  \best{32.52} &     \nbest{58.33} &         32.41 & \nbest{41.34} &         22.83 &         17.75 &         13.87 &             83.53 &         11.02 &             88.05 &         14.55 &             82.28 \\ 
BEiT-L-384 &  \best{1.53} &  \best{3.91} & \nbest{6.91} & \nbest{55.60} &  \best{12.78} &  \best{20.37} &         14.39 &         17.75 & \nbest{32.57} &      \best{58.73} &  \best{30.21} &         41.22 &  \best{21.76} &  \best{18.92} &  \best{13.53} &      \best{84.65} &   \best{9.63} &      \best{91.05} &  \best{13.60} &      \best{85.81} \\ 
\midrule
No Aug &         3.68 &         0.00 &         6.39 &  \best{56.55} &         17.12 &         14.28 &         21.54 &          9.85 &         35.62 &             52.92 &         35.38 &  \best{39.54} &         24.90 &         15.88 & \nbest{16.69} &             76.55 &         14.41 &             80.27 &         17.50 &             76.18 \\ 
ColorJitter &         3.00 &         1.30 &  \best{6.31} & \nbest{56.38} & \nbest{16.95} &         14.36 &         19.72 &         10.71 &         35.65 &             53.08 & \nbest{35.16} &         38.73 &  \best{24.47} & \nbest{16.16} &  \best{16.63} &      \best{76.93} &         14.25 &             80.59 &         17.58 &             75.62 \\ 
 CutOut &         3.68 &         1.55 &         6.51 &         55.93 &         17.25 &         14.35 & \nbest{18.98} &  \best{11.86} &         35.73 &             52.81 &         35.75 &         38.86 &         25.17 &         15.92 &         16.71 &     \nbest{76.61} &         14.09 &             80.76 &         17.43 &             75.86 \\ 
   RandAugment & \nbest{2.37} & \nbest{2.09} & \nbest{6.36} &         56.34 &  \best{16.89} &  \best{14.61} &         19.25 &         11.05 &  \best{35.36} &     \nbest{53.30} &  \best{34.11} & \nbest{39.40} &         24.82 &         15.83 &         16.91 &             76.34 & \nbest{13.98} &     \nbest{81.16} &  \best{16.98} &      \best{76.65} \\ 
    All &  \best{2.26} &  \best{2.97} &         6.36 &         56.30 &         17.09 & \nbest{14.36} &  \best{17.17} & \nbest{11.66} & \nbest{35.52} &      \best{53.44} &         35.41 &         39.12 & \nbest{24.58} &  \best{16.31} &         16.80 &             76.54 &  \best{13.61} &      \best{81.96} & \nbest{17.08} &     \nbest{76.48} \\ 
    \midrule
Base & \nbest{2.47} & \nbest{0.00} &  \best{6.49} &  \best{55.87} &         16.62 &         14.95 & \nbest{18.59} & \nbest{12.09} & \nbest{35.15} &     \nbest{54.00} &         36.01 &  \best{39.42} & \nbest{24.69} &  \best{16.20} &         16.44 &             77.08 &         13.52 &             82.54 &         16.87 &     \nbest{77.22} \\ 
 No Kitti &         3.05 &       -14.82 &        17.98 &         23.73 &  \best{16.02} &  \best{15.57} &         21.42 &         10.85 &         36.04 &             52.89 & \nbest{34.93} & \nbest{39.39} &         27.32 &         14.50 &         16.41 &             77.35 & \nbest{13.19} &     \nbest{83.43} &  \best{16.36} &      \best{78.12} \\ 
  No Mannequin &         3.89 &       -12.62 &         6.83 &         55.20 &         24.42 &          9.12 &  \best{17.07} &         11.60 &         35.73 &             53.12 &         37.04 &         33.11 &  \best{24.67} &         15.95 &         17.87 &             73.60 &         18.36 &             70.35 &         22.49 &             63.12 \\ 
 No \acl{stv} &         3.79 &        -8.87 &         7.15 &         54.72 &         16.51 &         14.59 &         30.15 &          6.43 &         36.48 &             51.85 &         35.85 &         37.47 &         27.07 &         13.92 & \nbest{16.30} &     \nbest{77.67} &         13.65 &             82.62 &         17.13 &             77.20 \\ 
With \acl{ctv} &  \best{1.79} &  \best{0.58} & \nbest{6.67} & \nbest{55.33} & \nbest{16.36} & \nbest{15.09} &         19.41 &  \best{12.59} &  \best{35.07} &      \best{54.25} &  \best{34.68} &         38.90 &         24.84 & \nbest{16.02} &  \best{16.12} &      \best{77.79} &  \best{12.76} &      \best{84.21} & \nbest{16.81} &             77.14 \\ 
% \midrule
% full no md2 & \nbest{1.89} & \nbest{0.00} & \nbest{9.00} & \nbest{53.50} &  \best{16.89} &  \best{14.66} & \nbest{23.57} & \nbest{11.13} & \nbest{35.99} &     \nbest{52.70} & \nbest{35.33} & \nbest{38.15} & \nbest{25.47} & \nbest{15.73} & \nbest{17.91} &     \nbest{75.03} & \nbest{21.68} &     \nbest{71.41} & \nbest{17.69} &     \nbest{75.67} \\ 
%    full md2 &  \best{1.11} &  \best{7.01} &  \best{6.50} &  \best{55.62} & \nbest{16.96} & \nbest{14.48} &  \best{18.49} &  \best{11.64} &  \best{35.62} &      \best{52.95} &  \best{34.97} &  \best{38.83} &  \best{24.44} &  \best{16.25} &  \best{16.85} &      \best{76.50} &  \best{14.27} &      \best{80.54} &  \best{17.23} &      \best{76.23} \\
% \midrule
% kitti no learn K &  \best{1.47} &   \best{0.00} &  \best{7.19} & \nbest{54.70} &  \best{29.94} &  \best{7.06} &  \best{27.56} &  \best{5.46} & \nbest{41.12} &     \nbest{41.98} &  \best{40.75} &  \best{27.82} & \nbest{27.42} & \nbest{12.74} & \nbest{19.67} &     \nbest{69.58} & \nbest{20.88} &     \nbest{63.03} &  \best{25.39} &      \best{58.44} \\ 
%    kitti learn K & \nbest{1.53} & \nbest{-0.34} & \nbest{7.23} &  \best{55.05} & \nbest{30.12} & \nbest{6.72} & \nbest{28.21} & \nbest{5.27} &  \best{41.04} &      \best{42.34} & \nbest{41.50} & \nbest{27.08} &  \best{26.81} &  \best{13.43} &  \best{19.58} &      \best{69.81} &  \best{20.58} &      \best{63.61} & \nbest{25.73} &     \nbest{57.83} \\ 
% \midrule
% mc no learn K & \nbest{1.89} & \nbest{0.00} & \nbest{21.65} & \nbest{16.27} & \nbest{16.66} & \nbest{14.20} &  \best{23.93} &  \best{9.17} & \nbest{37.61} &     \nbest{50.26} & \nbest{36.21} & \nbest{36.72} & \nbest{31.61} & \nbest{11.83} & \nbest{16.98} &     \nbest{76.52} & \nbest{14.11} &     \nbest{80.96} & \nbest{16.36} &     \nbest{78.11} \\ 
%    mc learn K &  \best{1.11} &  \best{2.00} &  \best{21.31} &  \best{18.63} &  \best{16.12} &  \best{14.77} & \nbest{26.25} & \nbest{8.93} &  \best{37.10} &      \best{51.11} &  \best{35.49} &  \best{37.88} &  \best{31.32} &  \best{11.93} &  \best{16.59} &      \best{77.18} &  \best{13.15} &      \best{83.38} &  \best{16.13} &      \best{78.64} \\
\bottomrule
\end{tabular}
\end{adjustbox}

\emph{%
Highlighted cells are \emph{\textbf{NOT zero-shot}} results.
\textbf{S}=Stereo, \textbf{M}=Monocular, \textbf{D}=Ground-truth Depth.
}


% \mycaption{Leave-one-out Ablation}{%
% We study the contribution of each proposed component. 
% Randomizing the support frames, learning camera parameters and augmenting the image shape all contribute to improving overall performance. 
% }

% \begin{tabular}{@{}llllllllllll@{}}
% \toprule
%                             & \multicolumn{2}{c}{\textbf{Multi-task}} &           \multicolumn{3}{c}{\textbf{\acl{kez}}} &             \multicolumn{3}{c}{\textbf{\acs{mc}}} & \multicolumn{3}{c}{\zs\textbf{\acs{syns} (Val)}} \\ 
%                                                             \cmidrule(lr){2-3}                                  \cmidrule(lr){4-6}                                \cmidrule(lr){7-9} \cmidrule(lr){10-12}
%                             & R\down & \acs{relimp}\up &  Rel\down &          F\up & \acs{d25}\up &      Rel\down &          F\up & \acs{d25}\up &      Rel\down &          F\up & \acs{d25}\up \\ 
% \midrule
%   \textbf{Full} &  \best{2.20} &   \best{0.00} & \nbest{6.16} & \nbest{57.60} &     \nbest{95.52} &         14.39 &         17.67 &     \nbest{82.23} & \nbest{20.34} &         17.08 &      \best{69.88} \\ 
% \midrule
%                   Fwd \acs{Pose} &         2.60 & \nbest{-0.08} &         6.18 &         57.47 &             95.47 &         14.36 &         17.52 &             82.22 &  \best{20.24} &  \best{17.20} &             69.52 \\ 
% $\acs{offset} = \pm1$ & \nbest{2.30} &         -0.60 &  \best{6.03} &  \best{58.23} &      \best{95.67} &  \best{14.17} &  \best{17.92} &      \best{82.43} &         21.04 &         16.04 &             68.33 \\ 
%             Fixed \acs{Cam} &         4.00 &         -1.46 &         6.30 &         56.93 &             95.38 &         14.95 &         17.11 &             81.00 &         20.46 & \nbest{17.11} &     \nbest{69.56} \\ 
%               No \ac{araug} &         4.50 &         -4.72 &         7.42 &         52.89 &             93.99 & \nbest{14.32} & \nbest{17.87} &             82.16 &         21.32 &         16.10 &             67.64 \\ 
%                        None &         5.40 &         -5.52 &         7.47 &         51.83 &             94.19 &         14.62 &         17.01 &             81.29 &         21.21 &         16.72 &             67.03 \\ 
% \bottomrule
% \end{tabular}

% \emph{%
% Highlighted cells indicate \emph{\textbf{zero-shot}} results.
% }



==> Tables/res_reloc.tex <==
% MapFreeReloc benchmark results.

\mycaption{Map-free Relocalization~\cite{Arnold2022}}{%
% See \sct{res:reloc} for details.
We incorporate \acs{kbr} into a feature-matching pipeline for singe-image relocalization. 
We once again outperform the \acl{ssmde} baselines in every metric and perform on par with supervised \ac{sota}.
% This demonstrates the applicability to downstream real-world tasks.
}

\begin{tabular}{@{}lllllllll@{}}
\toprule
                              &       &                                    \multicolumn{4}{c}{Pose} &                       \multicolumn{3}{c}{VCRE} \\
                                                                                 \cmidrule(lr){3-6}                               \cmidrule(lr){7-9}
                              & Train &   Trans\down &      Rot\down &         P\up &        AUC\up &     Error\down &          P\up &        AUC\up \\
\midrule
         Garg~\cite{Garg2016} &     S &         2.96 & \nbest{52.57} &         5.43 &         17.15 &         188.20 &         24.84 & \nbest{51.61} \\ 
 Monodepth2~\cite{Godard2017} &    MS &         2.95 &         52.92 &         5.50 &         17.22 &         189.67 &         24.38 &         50.63 \\ 
      DiffNet~\cite{Zhou2021} &    MS &         2.97 &         53.19 &         5.65 &         17.71 &         188.80 &         24.78 &         51.24 \\ 
      HR-Depth~\cite{Lyu2021} &    MS & \nbest{2.94} &         52.95 & \nbest{5.67} & \nbest{17.95} & \nbest{187.83} & \nbest{25.06} &         51.52 \\ 
\midrule
    \textbf{\acs{kbr} (Ours)} &     M &  \best{2.63} &  \best{49.01} & \best{11.54} &  \best{32.02} &  \best{181.21} &  \best{29.96} &  \best{58.89} \\ 
\midrule
\midrule
      MiDaS~\cite{Ranftl2020} &     D &         2.60 &         46.92 & \nbest{11.39} &         30.44 & \nbest{180.64} &         30.45 &         59.72 \\ 
    DPT-ViT~\cite{Ranftl2021} &     D & \nbest{2.56} & \nbest{45.62} &         11.27 & \nbest{30.92} &         181.34 & \nbest{30.60} & \nbest{60.03} \\ 
   DPT-BEiT~\cite{Ranftl2021} &     D &  \best{2.49} &  \best{44.99} &  \best{12.56} &  \best{32.48} &         181.67 &  \best{32.46} &  \best{62.03} \\ 
    NeWCRFs~\cite{Weihao2022} &     D &         2.89 &         51.92 &          6.69 &         20.77 &         184.63 &         25.89 &         52.93 \\ 
\midrule 
   DPT-NYUD~\cite{Arnold2022} &  D+FT &         2.67 &         47.66 &          9.17 &         26.46 &         184.53 &         28.68 &         56.87 \\ 
  DPT-Kitti~\cite{Arnold2022} &  D+FT &         2.66 &         49.21 &         10.86 &         29.99 &  \best{178.49} &         28.37 &         56.86 \\ 
\bottomrule
\end{tabular}

\emph{%
\textbf{Trans}=meters, \textbf{Rot}=deg, \textbf{VCRE}=px, \textbf{Precision}=\%, \textbf{AUC}=\%.
}


==> Tables/resources.tex <==
% Model params & FPS.

\mycaption{Model Complexity}{%
\acs{kbr} retains the architecture from Monodepth Benchmark~\cite{Spencer2022}, while \acs{kbr++} matches \acs{dpt-beit}~\cite{Ranftl2021}.
Despite being of equivalent complexity, our models greatly outperforms the \ac{ssl} baselines and can close the gap to supervised performance. 
}

\begin{tabular}{@{}llllll@{}}
\toprule
                             & Backbone                     & MParam\down    & FPS\up        \\
\midrule 
\textbf{\acs{kbr} (Ours)~\cite{Spencer2023c}}    & ConvNeXt-B~\cite{Liu2022}    & \best{92.65}   & \best{61.50}  \\
\textbf{\acs{kbr++} (Ours)}  & BEiT-L~\cite{Bao2022}        & 345.01         & 9.60          \\
\midrule
MiDaS~\cite{Ranftl2020}      & ResNeXt-101~\cite{Xie2017}   & \nbest{105.36} & \nbest{51.38} \\
DPT~\cite{Ranftl2021}        & ViT-L~\cite{Dosovitskiy2021} & 344.06         & 14.54         \\
DPT~\cite{Ranftl2021}        & BEiT-L~\cite{Bao2022}        & 345.01         & 9.60          \\
NeWCRFs~\cite{Yuan2021}      & Swin~\cite{Liu2021b}         & 270.44         & 21.61         \\
\bottomrule
\end{tabular}

==> Tables/supp_learnk.tex <==

% \footnotesize

\mycaption{Learning Camera Intrinsics}{%
Performance when training on a single dataset (Kitti or \acl{mc}) and learning camera intrinsics. 
If the cameras are not perfectly calibrated, learning the intrinsics can improve accuracy. 
}

\begin{tabular}{@{}lllllll@{}}
\toprule
              &    \multicolumn{3}{c}{\textbf{\acl{kez}}} \\ 
              \cmidrule(lr){2-4}  
              &     Rel\down &          F\up & $\delta_{.25}$\up    \\ 
\midrule
     Baseline  & \nbest{5.69} &  \best{60.88} &     \nbest{95.89}  \\ 
Learn \acs{Cam} &  \best{5.68} & \nbest{60.81} &      \best{95.90} \\ 
\bottomrule
\end{tabular}
\quad
\begin{tabular}{@{}lllllll@{}}
\toprule
              &     \multicolumn{3}{c}{\textbf{\acs{mc}}} \\ 
              \cmidrule(lr){2-4}  
                &      Rel\down &          F\up & $\delta_{.25}$\up \\ 
\midrule
     Baseline   & \nbest{16.66} & \nbest{14.20} &     \nbest{77.18} \\ 
Learn \acs{Cam} &  \best{16.12} &  \best{14.77} &      \best{78.40} \\ 
\bottomrule
\end{tabular}


==> Tables/supp_motion.tex <==

\scriptsize
\addtolength{\tabcolsep}{0.05em}
\def\mc{\multicolumn}


\mycaption{Monodepth2~\cite{Godard2019} Losses}{%
The minimum reconstruction loss and automasking from Monodepth2 serve as valuable proxies to increase robustness to dynamic objects, while remaining simple and efficient. 
}


\begin{tabular}{@{}lllllllllllllllllllll@{}}
\toprule
                             & \mc{2}{c}{\textbf{Multi-task}} & \mc{2}{c}{\bf\acs{keb}}            & \mc{2}{c}{\bf\acs{mc}}             & \mc{2}{c}{\bf\acs{ddad}}      & \mc{2}{c}{\bf\acs{dio}}       & \mc{2}{c}{\bf\acs{sintel}}    & \mc{2}{c}{\bf\acs{syns}}      & \mc{2}{c}{\bf\acs{dii}}       & \mc{2}{c}{\bf\acl{nyud}}          & \mc{2}{c}{\bf\acs{tum}}       \\  
                                       \cmidrule(lr){2-3}                   \cmidrule(lr){4-5}                   \cmidrule(lr){6-7}              \cmidrule(lr){8-9}             \cmidrule(lr){10-11}            \cmidrule(lr){12-13}            \cmidrule(lr){14-15}            \cmidrule(lr){16-17}                \cmidrule(lr){18-19}  \cmidrule(lr){20-21}
                             &   \acs{rank}\down &        \acs{relimp}\up &        Rel\down &             F\up &         Rel\down &            F\up &      Rel\down &          F\up &      Rel\down &  \acs{d25}\up &      Rel\down &          F\up &      Rel\down &          F\up &      Rel\down &  \acs{d25}\up &       Rel\down &     \acs{d25}\up &      Rel\down &  \acs{d25}\up \\
\midrule
         Baseline & \nbest{1.89} & \nbest{0.00} & \nbest{9.00} & \nbest{53.50} &  \best{16.89} &  \best{14.66} & \nbest{23.57} & \nbest{11.13} & \nbest{35.99} &     \nbest{52.70} & \nbest{35.33} & \nbest{38.15} & \nbest{25.47} & \nbest{15.73} & \nbest{17.91} &     \nbest{75.03} & \nbest{21.68} &     \nbest{71.41} & \nbest{17.69} &     \nbest{75.67} \\ 
MinRec+Automask &  \best{1.11} &  \best{7.01} &  \best{6.50} &  \best{55.62} & \nbest{16.96} & \nbest{14.48} &  \best{18.49} &  \best{11.64} &  \best{35.62} &      \best{52.95} &  \best{34.97} &  \best{38.83} &  \best{24.44} &  \best{16.25} &  \best{16.85} &      \best{76.50} &  \best{14.27} &      \best{80.54} &  \best{17.23} &      \best{76.23} \\ 
\bottomrule
\end{tabular}


==> Tables/supp_res.tex <==
% Supplementary results using median scaling. 

\addtolength{\tabcolsep}{0.2em}
\def\mc{\multicolumn}

\mycaption{Median-Scaling Results}{%
This represents the common \ac{ssmde} evaluation procedure~\cite{Zhou2017}. 
Removing the shift alignment reduces performance for all approaches. 
Our method still outperforms all existing \acl{ssmde} models, and \ac{crf} in many cases.
}


\begin{tabular}{@{}llllllllllllllllllll@{}}
\toprule
                             &       & \mc{4}{c}{\bf In-Distribution}                                         & \mc{8}{c}{\bf Outdoor}                                                                                                        & \mc{6}{c}{\bf Indoor}                                                                            \\
                                       \cmidrule(lr){3-6}                                                       \cmidrule(lr){7-14}                                                                                                             \cmidrule(lr){15-20}
                             &       & \mc{2}{c}{\bf\acs{keb}}            & \mc{2}{c}{\bf\acs{mc}}            & \mc{2}{c}{\bf\acs{ddad}}      & \mc{2}{c}{\bf\acs{dio}}       & \mc{2}{c}{\bf\acs{sintel}}    & \mc{2}{c}{\bf\acs{syns}}      & \mc{2}{c}{\bf\acs{dii}}       & \mc{2}{c}{\bf\acl{nyud}}         & \mc{2}{c}{\bf\acs{tum}}       \\  
                                       \cmidrule(lr){3-4}                   \cmidrule(lr){5-6}                  \cmidrule(lr){7-8}              \cmidrule(lr){9-10}             \cmidrule(lr){11-12}            \cmidrule(lr){13-14}            \cmidrule(lr){15-16}            \cmidrule(lr){17-18}               \cmidrule(lr){19-20}
                             & Train &        Rel\down &             F\up &        Rel\down &            F\up &      Rel\down &          F\up &      Rel\down &  \acs{d25}\up &      Rel\down &          F\up &      Rel\down &          F\up &      Rel\down &  \acs{d25}\up &       Rel\down &    \acs{d25}\up &      Rel\down &  \acs{d25}\up \\
\midrule
Garg~\cite{Garg2016}         & S     & \zs\nbest{7.65} & \zs\nbest{53.28} & \nbest{34.55} & \nbest{9.29} &         26.77 &         4.77 &         57.87 &             42.85 & \nbest{53.16} & \nbest{30.98} &         31.68 &         13.58 &         30.63 &             51.00 &         26.78 &             54.29 & \nbest{27.37} &     \nbest{55.26} \\
Monodepth2~\cite{Godard2019} & MS    &  \zs       7.90 &   \zs      50.50 &         35.88 &         8.18 &         25.46 &         4.77 &         57.61 &             43.21 &         54.40 &         30.11 &         30.05 &         13.28 &         33.51 &             47.49 &         29.87 &             50.08 &         30.59 &             49.82 \\
DiffNet~\cite{Zhou2021}      & MS    &  \zs       7.98 &   \zs      49.60 &         35.50 &         8.15 &         24.17 &         4.75 & \nbest{55.68} &     \nbest{45.37} &         55.23 &         29.44 & \nbest{29.75} &         13.41 & \nbest{28.67} &     \nbest{53.82} & \nbest{26.62} &     \nbest{54.69} &         28.56 &             53.07 \\
HR-Depth~\cite{Lyu2021}      & MS    &  \zs       7.70 &   \zs      51.49 &         35.89 &         8.62 & \nbest{24.01} & \nbest{5.08} &         57.88 &             43.92 &         53.91 &         30.89 &         29.87 & \nbest{14.03} &         32.88 &             47.67 &         27.32 &             53.06 &         29.22 &             52.31 \\
\midrule
\textbf{\acs{kbr} (Ours)}    & M     &  \zs\best{7.23} &  \zs\best{54.63} &  \zs\best{18.73} & \zs\best{15.04} &  \best{14.01} & \best{14.01} &  \best{43.80} &      \best{60.84} &  \best{37.06} &  \best{36.01} &  \best{24.92} &  \best{16.49} &  \best{18.88} &      \best{72.09} &  \best{13.27} &      \best{83.65} &  \best{16.60} &      \best{76.48} \\
\midrule
\midrule
MiDaS~\cite{Ranftl2020}      & D     &         18.45 &         20.13 & \nbest{26.02} &         10.61 &         18.38 &          8.28 &  \best{48.63} &      \best{60.15} &  \best{39.09} &  \best{32.72} &         35.30 &          9.18 & \nbest{18.08} &     \nbest{74.48} & \nbest{23.11} &     \nbest{69.67} & \nbest{17.75} &             76.99 \\ 
DPT-ViT~\cite{Ranftl2021}    & D     & \nbest{14.23} &         36.25 &         28.54 &         11.38 &         17.83 &          8.99 &         72.46 &             49.09 &        128.86 &         29.58 &         32.69 &         12.93 &         36.82 &             55.15 &         24.82 &             67.95 &         24.33 &             78.16 \\ 
DPT-BEiT~\cite{Ranftl2021}   & D     &  \zs       18.20 & \zs\nbest{37.46} &         30.79 & \nbest{12.58} & \nbest{15.39} & \nbest{11.78} &         70.30 &             50.03 &         60.20 &         29.54 & \nbest{31.09} & \nbest{13.76} &         51.07 &             53.11 &    \zs     75.32 &   \zs          42.91 &         25.27 &      \best{83.07} \\ 
NeWCRFs~\cite{Weihao2022}    & D     &  \zs \best{5.55} & \zs \best{56.45} &  \best{22.15} &  \best{13.68} &  \best{11.87} &  \best{13.44} & \nbest{50.52} &     \nbest{51.16} & \nbest{48.42} & \nbest{32.30} &  \best{27.79} &  \best{14.50} &  \best{16.15} &      \best{79.52} &   \zs\best{7.00} &   \zs   \best{94.44} &  \best{14.93} &     \nbest{80.63} \\ 
\bottomrule
\end{tabular}

\emph{%
Highlighted cells are \emph{\textbf{NOT zero-shot}} results.
\textbf{S}=Stereo, \textbf{M}=Monocular, \textbf{D}=Ground-truth Depth.
}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
